I-BERT: Integer-only BERT Quantization

Transformer based models, like BERT and RoBERTa, have achieved state-of-the-art results in many Natural Language Processing tasks. However, their memory footprint, inference latency, and power consumption are prohibitive efficient inference at the edge, and even at the data center. While quantization can be a viable solution for this, previous work on quantizing Transformer based models use floating-point arithmetic during inference, which cannot efficiently utilize integer-only logical units such as the recent Turing Tensor Cores, or traditional integer-only ARM processors. In this work, we propose I-BERT, a novel quantization scheme for Transformer based models that quantizes the entire inference with integer-only arithmetic. Based on lightweight integer-only approximation methods for nonlinear operations, e.g., GELU, Softmax, and Layer Normalization, I-BERT performs an end-to-end integer-only BERT inference without any floating point calculation. We evaluate our approach on GLUE downstream tasks using RoBERTa-Base/Large. We show that for both cases, I-BERT achieves similar (and slightly higher) accuracy as compared to the full-precision baseline. Furthermore, our preliminary implementation of I-BERT shows a speedup of 2.4-4.0x for INT8 inference on a T4 GPU system as compared to FP32 inference. The framework has been developed in PyTorch and has been open-sourced.

==> _s5_discussion.tex <==


\section{\textbf{Ablation Study}}
\label{sec:ablation_study}


% --------------------------------------------------------
In this section, we empirically validate i-GELU, our approximation method for GELU. 
For comparison, we implement two variants of \OURS by replacing i-GELU with GELU and h-GELU respectively.
Note that the former is the exact computation of GELU with floating point arithmetic 
and the later is another integer-only approximation method for GELU (see~\sref{sec:methodology}).
We use RoBERTa-Large model as baseline, and we use QNLI, SST-2, MPRC, and RTE for downstream tasks. 
All models are trained and fine-tuned according to the procedure described in~\sref{sec:results}.
We report the accuracy in~\tref{tab:gelu_comparison}.

As one can see in the table, replacing GELU with h-GELU approximation results in accuracy degradation for all downstream tasks except for MRPC.
Accuracy drops by 0.5 on average and up to 1.1 for RTE task.
Although accuracy slightly improves for MRPC, the amount of increase is smaller than replacing GELU with i-GELU.
This empirically demonstrates that h-GELU is not sufficiently tight enough to approximate GELU well.
Interestingly, approximating GELU with i-GELU results in strictly better accuracy for all four downstream tasks than approximating GELU with h-GELU.
i-GELU outperforms h-GELU by 0.7 on average, and it achieves comparable or slightly better result to the non-approximated full-precision GELU. 
This implies that i-GELU allows tighter approximation for GELU, as compared to h-GELU.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
\caption{ 
Accuracy of models that use GELU, h-GELU and i-GELU for GELU computation. Note that the former is the full-precision, floating point computation while the latter two are the integer-only approximations. 
}

\vskip 0.1in
\label{tab:gelu_comparison}
    \centering
    \small{
    \setlength{\tabcolsep}{5pt}{
    \centerline{
       \begin{tabular}{lccccccc}
        \toprule
        \ha         & Int-only & QNLI & SST-2    & MRPC     & RTE  & Avg.    \\ 
        \midrule
        \ha GELU    & \xmark            & 94.4      & 96.3          & 92.6          & 85.9      & 92.3 \\
        \ha h-GELU  & \cmark            & 94.3      & 96.0          & 92.8          & 84.8      & 92.0 \\
        \midrule
        \hc i-GELU  & \cmark            & \tb{94.5} & \tb{96.4}     & \tb{93.0}     & \tb{87.0} &  \tb{92.7} \\
        \bottomrule
        \end{tabular} 
    }
    }
    }
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
